Computation of covariant lyapunov vectors using data assimilation

Computing Lyapunov vectors from partial and noisy observations is a challenging problem. We propose a method using data assimilation to approximate the Lyapunov vectors using the estimate of the underlying trajectory obtained from the filter mean. We then extensively study the sensitivity of these approximate Lyapunov vectors and the corresponding Oseledets' subspaces to the perturbations in the underlying true trajectory. We demonstrate that this sensitivity is consistent with and helps explain the errors in the approximate Lyapunov vectors from the estimated trajectory of the filter. Using the idea of principal angles, we demonstrate that the Oseledets' subspaces defined by the LVs computed from the approximate trajectory are less sensitive than the individual vectors.

==> 3_methodology-unused.tex <==
\subsection{Covariant and Backward Lyapunov Vector}
CLVs derive their name from their most important property of being covariant under the tangent linear equations. They are norm-independent and time invariant local basis vectors in the tangent space along which perturbations grows or decays along the trajectory with the associated rates being the lyapunov exponents i.e. an infinitesimal error along $i^{th}$ CLV grows with $exp(\lambda_i t)$ forward in time and decays as $exp(-\lambda_i t)$ backwards in time, $\lambda_i $ being the $i^{th}$ lyapunov exponent(\cite{Diego(2008)},\cite{Yang(2009)}).
The backward lyapunov vectors or BLVs are obtained as consequence of the Benettin's algorithm, which denote the directions in the tangent space along which the errors 

Ginelli's algorithm computes CLVs given a dynamical model with it's tangent linear equations while also computing BLVs as an intermediate step. It requires a trajectory with a sufficiently long forward transient and an additional backward transient in order to converge to the BLVs and the CLVs respectively. After the forward transient, the forward gram-schmidt converges to the BLVs. From this point, the BLVs $G_n$ and their growth rates are stored at the time steps over the interval of sampling denoted as $R_{n,n-1}$, which are the result of QR-decomposition applied for the gram-schmidt re-orthonormalization procedure. The procedure continues over the sampling interval and the backward interval. At the end of the backward interval, a generic non-singular upper triangular martix $\tilde C$is initialized and evolved using the growth rate matrix previously stored duing the forward evolution.
This is motivated by the fact that the $i^{th}$ CLV lie in the span of first $i$-BLVs, hence the upper triangular traingular structure.
These coefficient matrices are then computed backwards in time via equation \ref{eq-backward}.
These coefficient matrices are then store after the backward transient is over, the CLVs are then expressed in the basis of BLVs.
The two sets of matrices stored, one containing the BLVs at the time instants in the sampling interval, and the other being the co-efficient matrices $C_n$, which can be used to get the CLVs at any time $n$ using the following relation
\begin{equation}
V_n=G_n C_n    
\end{equation}

\subsection{Ensemble Kalman Filters}
Introduced in the data assimilation community by G. Evensen \cite{Evensen(2003)}, ensemble kalman filters are a Monte-Carlo approach of approximation of the original Kalman filter which is a sequential state estimation algorithm \cite{Cohn(1997)} based on the assumption of linearity and gaussianity of the probability distributions involved to recursively compute from the prior distribution, the posterior distribution incorporating the latest observation by simply updating mean and covariance. The filter employs ensemble representation of probability distributions which is a collection states sampled from the respective pdfs. This approach is particularly useful when the dynamics is nonlinear as each ensemble member can be integrated individually. In between the observations, each member of the ensemble is evolved in time according to the model equations. When new observation arrives, the mean and covariance required in the bayesian update is replaced by the empirical mean and covariance computed from the ensemble respectively. Localization and inflation are ad-hoc methods which makes EnKF work with small ensemble size, making it feasible for systems with large dimensions and a practical choice for operational data assimilation \citep{Carrassi(2018)}. We use EnKF for performing twin experiment with Lorenz-96 model using noisy and partial observations to assimilate and obtain analysis trajectory.
The analysis trajectory is further used in the calculation of BLVs and CLVs using $\hat x_t$ to evaluate the jacobian of evoving the perturbations whenever needed. In order to compare the obtained vectors, we also compute these vectors from the true underlying trajectory known to us in the numerical experiment.  

\subsection{Lyapunov Vectors from perturbed trajectory}
The estimates of the states computed from a data assimilation algorithm are near to the true state under some specific metric. At time t, the analysis mean obtained from a filter is the best estimate which takes into account all the observations up to that time. The sequence of analysis mean as states obtained over time is not a dynamical trajectory of the model but at any time t, the analysis mean lies close to the true state points in some truncated state space. Hence we propose to use the analysis mean of the above filter as a proxy for the true state of the system which can be used to obtain the lyapunov vectors along the trajectory the system is evolving. The above notion of sensitivity to the perturbations in base trajectory allows us to think of the analysis mean trajectory as a perturbed trajectory obtained from the true trajectory where the perturbations follow the error distribution of the analysis. This analysis mean is then used for evaluating the model jacobian, a crucial step in the calculation of the LVs. The estimated trajectory can be understood as a trajectory obtained by perturbing the true trajectory with a noise which is equivalent to the unknown error statistics of the difference between the true state and it's best estimate.      

To investigate the stability of numerically calculated LVs about the reference trajectory, we add noise to the orbit by adding random samples from a standard normal distribution of covariance $\sigma^2 \mathbf{I}$ at each point of the orbit. We refer to the obtained trajectory as perturbed orbit for the respective $\sigma$ value in future discussions. 
The calculation of BLVs over any interval requires only the forward transient which is required for the convergence of the BLVs. When using Ginelli's algorithm to compute CLV along a trajectory, we need both a forward and a backward transient interval in addition to the interval over which they are calculated, the details can be found in the paper (\cite{Ginelli(2013)}). We then compute all the BLVs and CLVs about the true and the perturbed trajectories over a common interval using the same forward and backward transient intervals. 

\subsection{Metric}\label{ssc-metric}
We compare the individual LVs from both the perturbed trajectory and the reconstructed trajectory with the ones derived from the true underlying trajectory.
To understand the sensitivity of the individual LVs with respect to the perturbation strength $\sigma$, we use the angle between the $i^{th}$ Lyapunov vector computed from the original trajectory and the perturbed trajectory. We plot the median of the angle computed over the sampling interval along with the error bars which represent the $25^{th}$ and $75^{th}$ percentile of the angles.

In high-dimensional spaces, we know information is often restricted to a low-dimensional subspace, a crucial feature in uncovering underlying signals. A subspace of dimension $k$ in $R^n$ admits an infinite number of possible basis vectors. Two sets of basis vectors span the same subspace if all the principal angles are zero, although the individual vectors are misaligned with each other. Such subspaces are uniquely described by projection matrices instead of the basis vectors themselves. To investigate the quality of subspaces we obtain from the approximate LVs, we study the relative orientation between the subspace spanned by the first n-BLVs computed from the true and the perturbed trajectory. Principal angles are a set of acute angles in increasing order which quantify the similarity between two subspaces by comparing the relative orientation of any two subspaces and identifying the directions in which they are most similar or most different. If two subspaces are of different dimensions, the number of the principal angles is equal to mininum dimension of the two subspaces.\\

Principal angles are defined as a sequence of minimum angles between two unit vectors corresponding to each of the two subspaces, such that the unit vectors are chosen to minimize the angle between them while being orthogonal to all the previous unit vectors obtained in their respective subspaces. Mathematically, if we have two subspaces $\mathcal{X}$ and $\mathcal{Y}$ whose orthogonal basis is available as columns of two matrices $X$ and $Y$ respectively, they are defined as by an m-tuple of angles,
$\theta(\mathcal{X},\mathcal{Y})=[\theta_1,\theta_2,..,\theta_m]$
where $\theta_k$ is defined as follows 
$$cos(\theta_k)= \max_{x \in \mathcal{X}} \max_{y \in \mathcal{Y}} |x^T y|, \text{ subject to } ||x||=||y||=1, x^Tx_i ,y^Ty_i, i=1,...,k-1$$

When the set of angles between two subspaces are all small, this suggests that the two subspaces are closely aligned and have a strong degree of similarity. On the other hand, if the angles are large, this implies that the subspaces are more dissimilar and have less overlap. There are several methods for calculating the principal angles between two subspaces, including the singular value decomposition (SVD) and the QR decomposition. The angles can be computed easily from the SVD of the matrix product $X^T$ and $Y$ $$X^TY=U\Sigma V^T$$ The cosines of the principal angles are the diagonal elements of the matrix $\Sigma$.
